Birds of a Feather Flock Together: A Close Look at Cooperation Emergence via Multi-Agent RL

How cooperation emerges is a long-standing and interdisciplinary problem. Game-theoretical studies on social dilemmas reveal that altruistic incentives are critical to the emergence of cooperation but their analyses are limited to stateless games. For more realistic scenarios, multi-agent reinforcement learning has been used to study sequential social dilemmas (SSDs). Recent works show that learning to incentivize other agents can promote cooperation in SSDs. However, we find that, with these incentivizing mechanisms, the team cooperation level does not converge and regularly oscillates between cooperation and defection during learning. We show that a second-order social dilemma resulting from the incentive mechanisms is the main reason for such fragile cooperation. We formally analyze the dynamics of second-order social dilemmas and find that a typical tendency of humans, called homophily, provides a promising solution. We propose a novel learning framework to encourage homophilic incentives and show that it achieves stable cooperation in both SSDs of public goods and tragedy of the commons.

==> backup.tex <==
Reinforcement learning (RL) methods towards decision-making problems have received extensive attention and rapid development in the past decade. In combination with deep learning, state-of-the-art RL algorithms have proved effective in various complex domains of massive scales, including the single-agent game of Go ({\color{red}Silver et al., 2016}), and multi-agent games like Dota ({\color{red}OpenAI, 2018}) and StarCraft II ({\color{red}Vinyals et al., 2017}). However, as the problem increases in scale, and the network structure becomes more complicated, the training of RL models is increasingly time-consuming --- in practice, despite the acceleration via GPUs, the training of a single-agent model generally takes days or even weeks. The situation is even worse in multi-agent settings. {\color{red} ADD EXAMPLES} As the training gradually becomes the major bottleneck for multi-agent RL research, it seems inevitable to turn to parallelism for further acceleration, which is referred to as distributed RL.


Research on single-agent distributed RL algorithms has made much progress, but there is still little literature on its multi-agent counterpart. In this paper, we propose a general architecture for distributed multi-agent RL, which has such desirable properties as \textit{time-efficiency} (training completes in a reasonably short time), \textit{scalability} (training cost grows moderately as the scale increases), \textit{asynchrony} (training procedure is performed in parallel on multiple devices), and \textit{high throughput} (multiple actors sample experience in abundance and in parallel). Scalability is crucial to a practical distributed algorithm --- real-life problems may differ in scale (number of agents, size of action space, etc.), and training devices may vary greatly (with regard to computational power and device heterogeneity) as well; however, a successful algorithm is expected to yield asymptotically good performance in all settings. Parallelism is a natural approach for scalability, which in turn requires the algorithm to be asynchronized and of high throughput, in the sense that multiple actors who sample experiences from the environment could function independently from the learner. The same idea has been widely applied in single-agent distributed RL algorithms ({\color{red} GORILA, Ape-X, etc.}).

To adapt the isolated actor-learner architecture for multi-agent settings, several challenges posed by the intrinsic discrepancies between single- and multi-agent RL must be addressed. The first challenge is that the inference step of an actor is much more expensive in multi-agent settings, since the value functions of all agents should be calculated using the network. To accelerate the inference step, we shall allow actors to run on both CPUs and GPUs, and transfer as many actors to GPU as possible. This approach helps to make the most efficient and most flexible use of existing devices.

The second challenge roots in the sampling policy of the replay buffer. As past experiences differ in their potential contributions to the training, higher sampling priority should be assigned to more important experiences to further accelerate training ({\color{red}Schaul et al., 2016}). In single-agent settings, a replay buffer prioritized by current TD-error of the trajectory yield desirable performance ({\color{red}Ape-x}), where initial priority can be efficiently and precisely calculated by each actor. However, this is not directly feasible with multi-agent algorithms like QMIX, where TD-error calculation involves an extra mixing network that is quite expensive, and the calculation induces projection error by nature. Fortunately, approximations are acceptable, since initial priority only serves as a hint for sampling, and will be constantly updated during the training. In our architecture, newly-generated experiences are assigned the average priority in replay buffer, giving each of them a fair and moderate opportunity to be sampled at least once.

The third challenge is that the priorities of experiences in the replay buffer become largely inaccurate as the training proceeds, since accurate priorities are only updated when experiences get sampled by the learner, while the learner samples only a small proportion each time. The problem is even worsened due to approximated initial priorities. To keep the priorities up-to-date, we introduce priority-updater processes independent from the learner that constantly re-calculates priorities within the replay buffer.


Distributed single-agent RL algorithms have been a popular research area in recent years, among which the search for distributed value-based methods has been quite fruitful. The first pioneering value-based architecture, GORILA ({\color{red}Nair et al., 2015}), adapts the Deep Q-Network (DQN) for distributing acceleration. It introduces several innovative ideas, such as isolated actors and learners running in parallel, distributed neural networks, and distributed replay buffer storage, but is not widely used for poor time efficiency and sample efficiency caused by asynchronous SGD. Later, Ape-X ({\color{red}Horgan et al., 2018}) establishes the fundamental multiple-actor-single-learner architecture with a centralized replay buffer, and further improves the training performance via a replay buffer prioritized by trajectory TD-error ({\color{red}Schaul et al., 2016}), which yields state-of-the-art performance for Atari games. On top of Ape-X, R2D2 (Kapturowski et al., 2018) makes improvement by incorporating LSTM for better feature extraction, while SEED ({\color{red}Kapturowski et al., 2019}) features centralized inference interface within the learner module to reduce the cost of transmitting network weights frequently.

Another popular approach towards distributed single-agent RL is to adapt policy gradient methods to paralleled training. A3C (Mnih et al., 2016) first introduces a general asynchronous training architecture for actor-critic methods, in which workers retrieve network weights from a parameter server, independently interact with the environment to calculate gradients, and then send the gradients back to parameter server for centralized policy updates. DPPO (Heess et al., 2017) is the distributed implementation of PPO using a similar method of distributed gradient gathering. On the other hand, IMPALA (Espeholt et al., 2018) introduces an off-policy correction method (called the V-trace method), where the actor-learner architecture is utilized, and experience trajectories are communicated instead of gradients. Compared to A3C, it displays desirable properties of stabler convergence, better scalability and higher robustness.

Reinforcement learning in multi-agent settings is becoming increasingly important for complex real-world decision-making problems, and has been seeing significant progresses recently ({\color{red}MADDPG, QMIX, ROMA, etc.}). It is evident that the training of multi-agent RL generally takes more time and computational resources than that of single-agent RL, and thus distributing acceleration is more urgently demanded. Nevertheless, the demand is largely ignored, as hardly any existing literature has looked into the topic of distributed MARL architecture ({\color{red}2101.02308}). In this paper, we develop a novel architecture to address this challenge, which significantly improves the scalability of MARL algorithms.

==> improvement.tex <==


Our paper was submitted to ICML 2021 and got 3 weak accepts and 1 weak reject. The advantages of the paper were generally appreciated by the reviewers, including the importance of the problem, novelty, having good technical results, and being well-written. The reviewers thought, "The authors consider the second-order social dilemmas. This is quite innovative", "The 'didactic' example is quite clear and convincing," and "The proposed method is interesting and deserves attention." However, the reviewers didn't strongly argue for the acceptance of this paper due to the following concerns.

(1) The lack of a sensitivity analysis regarding the parameters used in the case study (Sec. 3).
(2) A formal treatment was expected to theoretically support the proposed method.
(3) Inaccuracies in reporting some of the related work. 
(4) The description of the method can be improved. 
(5) The lack of discussions of other possible solutions.

In this new version of our paper, we address these problems by

(1) Using a one-at-a-time method to analyze the sensitivity of the parameters and showing the results with a Tornado diagram in the paper. These results consolidate the robustness of our observations and claims across a wide range of conditions.
(2) Adding formal analyses for the case study, which provide insights into the proposed method and address the concern about theoretical grounding.
(3) Updating the references.
(4) Improving the presentation of our method, simplifying the notation to make it easier to understand.
(5) Discussing other possible solutions in Sec. 4.3 and clarifying the advantages of our method compared to other solutions. 

Beyond these suggested improvements, we restructure our case study to make it more concise and better motivate our solutions both empirically and formally.

We want to take this opportunity to express our gratitude to the ICML reviewers for their constructive comments. We also want to thank the NeurIPS reviewers in advance for their time and efforts that would be devoted to our submission.
